Kempe Swap K-Means: A Scalable Near-Optimal Solution for Semi-Supervised Clustering

This paper presents a novel centroid-based heuristic algorithm, termed Kempe Swap K-Means, for constrained clustering under rigid must-link (ML) and cannot-link (CL) constraints. The algorithm employs a dual-phase iterative process: an assignment step that utilizes Kempe chain swaps to refine current clustering in the constrained solution space and a centroid update step that computes optimal cluster centroids. To enhance global search capabilities and avoid local optima, the framework incorporates controlled perturbations during the update phase. Empirical evaluations demonstrate that the proposed method achieves near-optimal partitions while maintaining high computational efficiency and scalability. The results indicate that Kempe Swap K-Means consistently outperforms state-of-the-art benchmarks in both clustering accuracy and algorithmic efficiency for large-scale datasets.

==> tables/COL4/COL4_table_1.tex <==
\begin{table}[H]
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{cc|cccccc}
\toprule
\textbf{Dataset}                   & \textbf{Constraints Level} & \textbf{COPKM\_P} & \textbf{KSKM} & \textbf{KSKM\_E} & \textbf{BLPKMCC} & \textbf{PCCC} & \textbf{COPKM} \\ \midrule
\multirow{3}{*}{\textbf{banana}}   & \textbf{0.005}             & 1                 & 1             & 1                & 1                & 1             & 0              \\
                                   & \textbf{0.01}              & 1                 & 1             & 1                & 1                & 1             & 0              \\
                                   & \textbf{0.05}              & 1                 & 1             & 1                & 1                & 1             & 1              \\\hline
\multirow{3}{*}{\textbf{cifar10}}  & \textbf{0.005}             & 1                 & 1             & 1                & 1                & 1             & 1              \\
                                   & \textbf{0.01}              & 1                 & 1             & 1                & 1                & 1             & 0              \\
                                   & \textbf{0.05}              & 1                 & 1             & 1                & 1                & 1             & 1              \\\hline
\multirow{3}{*}{\textbf{cifar100}} & \textbf{0.005}             & 1                 & 1             & 1                & 1                & 1             & 1              \\
                                   & \textbf{0.01}              & 1                 & 1             & 1                & 0.5              & 0.5           & 1              \\
                                   & \textbf{0.05}              & 1                 & 1             & 1                & 0                & 0             & 0              \\\hline
\multirow{3}{*}{\textbf{letter}}   & \textbf{0.005}             & 1                 & 1             & 1                & 1                & 1             & 1              \\
                                   & \textbf{0.01}              & 1                 & 1             & 1                & 1                & 1             & 1              \\
                                   & \textbf{0.05}              & 1                 & 1             & 1                & 1                & 1             & 0              \\\hline
\multirow{3}{*}{\textbf{mnist}}    & \textbf{0.005}             & 1                 & 1             & 1                & 1                & 1             & 1              \\
                                   & \textbf{0.01}              & 1                 & 1             & 1                & 0.2              & 1             & 0              \\
                                   & \textbf{0.05}              & 1                 & 1             & 1                & 1                & 1             & 1              \\\hline
\multirow{3}{*}{\textbf{shuttle}}  & \textbf{0.005}             & 1                 & 1             & 1                & 1                & 1             & 1              \\
                                   & \textbf{0.01}              & 1                 & 1             & 1                & 1                & 1             & 1              \\
                                   & \textbf{0.05}              & 1                 & 1             & 1                & 1                & 1             & 1              \\ \bottomrule
\end{tabular}
}
\caption{Algorithm success rate among dataset collection 4.}
\label{tab:COL4_1}
\end{table}

==> tables/COL4/COL4_table_2.tex <==
\begin{table}[H]
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{cc|cccccc}
\toprule
\textbf{Dataset}                   & \textbf{Constraints Level} & \textbf{COPKM\_P} & \textbf{KSKM} & \textbf{KSKM\_E} & \textbf{BLPKMCC} & \textbf{PCCC} & \textbf{COPKM} \\ \midrule
\multirow{3}{*}{\textbf{banana}}   & \textbf{0.005}             & 6519.1            & 6482.97       & 6482.97          & 6482.98          & 6486.67       & -              \\
                                   & \textbf{0.01}              & 7707.22           & 7566.29       & 7566.29          & 7566.29          & 7567.65       & -              \\
                                   & \textbf{0.05}              & 10556.11          & 10556.11      & 10556.11         & 10556.11         & 10556.11      & 10556.11       \\ \hline
\multirow{3}{*}{\textbf{cifar10}}  & \textbf{0.005}             & 1.28E+08          & 1.27E+08      & 1.27E+08         & 1.27E+08         & 1.27E+08      & 1.28E+08       \\
                                   & \textbf{0.01}              & 1.47E+08          & 1.48E+08      & 1.47E+08         & 1.61E+08         & 1.57E+08      & -              \\
                                   & \textbf{0.05}              & 1.73E+08          & 1.73E+08      & 1.73E+08         & 1.73E+08         & 1.73E+08      & 1.73E+08       \\ \hline
\multirow{3}{*}{\textbf{cifar100}} & \textbf{0.005}             & 90808595          & 90710109      & 90708703         & 91217698         & 91012502      & 90817932       \\
                                   & \textbf{0.01}              & 93006014          & 92774481      & 92729305         & 94537010         & 93640143      & 92934055       \\
                                   & \textbf{0.05}              & 1.47E+08          & 1.47E+08      & 1.47E+08         & -                & -             & -              \\ \hline
\multirow{3}{*}{\textbf{letter}}   & \textbf{0.005}             & 124108            & 123274.5      & 123249.7         & 124061.7         & 123658.2      & 124320.1       \\
                                   & \textbf{0.01}              & 130686.3          & 129206.1      & 129009.4         & 129625.7         & 129235.8      & 130623.9       \\
                                   & \textbf{0.05}              & 208188            & 208140.5      & 208126           & 208124.3         & 208232.4      & -              \\ \hline
\multirow{3}{*}{\textbf{mnist}}    & \textbf{0.005}             & 43436555          & 43212644      & 43182717         & 43184195         & 43263288      & 43437504       \\
                                   & \textbf{0.01}              & 44631657          & 46145646      & 44423670         & 48776944         & 48542488      & -              \\
                                   & \textbf{0.05}              & 44514740          & 44514740      & 44514740         & 44514740         & 44514740      & 44514740       \\\hline
\multirow{3}{*}{\textbf{shuttle}}  & \textbf{0.005}             & 296049.2          & 293628.5      & 293946.3         & 305160.2         & 299481.9      & 296829.9       \\
                                   & \textbf{0.01}              & 330841.6          & 327093        & 328262.4         & 338035.9         & 331753.9      & 332760.9       \\
                                   & \textbf{0.05}              & 367447.7          & 366680.5      & 366680.5         & 366760.7         & 367244.7      & 367716.9       \\  \bottomrule
\end{tabular}
}
\caption{Algorithm clustering inertia among dataset collection 4.}
\label{tab:COL4_2}
\end{table}

==> tables/COL4/COL4_table_3.tex <==
\begin{table}[H]
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{cc|cccccc}
\toprule
\textbf{Dataset}                   & \textbf{Constraints Level} & \textbf{COPKM\_P} & \textbf{KSKM} & \textbf{KSKM\_E} & \textbf{BLPKMCC} & \textbf{PCCC} & \textbf{COPKM} \\ \midrule
\multirow{3}{*}{\textbf{banana}}   & \textbf{0.005}             & 0.37              & 0.12          & 0.14             & 1.94             & 4.73          & -              \\
                                   & \textbf{0.01}              & 0.18              & 0.21          & 0.34             & 2.5              & 5.22          & -              \\
                                   & \textbf{0.05}              & 0.03              & 0.02          & 0.02             & 1.55             & 0.08          & 0.03           \\\hline
\multirow{3}{*}{\textbf{cifar10}}  & \textbf{0.005}             & 55.18             & 523.56        & 594.81           & 1881.88          & 1224.33       & 16.07          \\
                                   & \textbf{0.01}              & 26.65             & 162.51        & 3603.56          & 3624.14          & 3633.96       & -              \\
                                   & \textbf{0.05}              & 2.63              & 7.55          & 9.24             & 1135.66          & 8.61          & 2.68           \\\hline
\multirow{3}{*}{\textbf{cifar100}} & \textbf{0.005}             & 620.46            & 1792.48       & 3588.09          & 3619.73          & 3638.03       & 166.84         \\
                                   & \textbf{0.01}              & 754.8             & 1345.87       & 3692.5           & 3949.69          & 3851.99       & 154.89         \\
                                   & \textbf{0.05}              & 28.41             & 362.72        & 3726.12          & -                & -             & -              \\\hline
\multirow{3}{*}{\textbf{letter}}   & \textbf{0.005}             & 2.73              & 41.08         & 102.57           & 571.06           & 749.37        & 6.77           \\
                                   & \textbf{0.01}              & 12.79             & 29.49         & 285.19           & 1002.48          & 695.34        & 5.47           \\
                                   & \textbf{0.05}              & 1.67              & 3.09          & 512.61           & 3376.45          & 1154.58       & -              \\\hline
\multirow{3}{*}{\textbf{mnist}}    & \textbf{0.005}             & 109.58            & 189.82        & 507.86           & 1805.8           & 804.6         & 12.76          \\
                                   & \textbf{0.01}              & 60.77             & 82.13         & 1304.47          & 3627.71          & 3790.51       & -              \\
                                   & \textbf{0.05}              & 2.02              & 2.82          & 3.36             & 1572.45          & 9.13          & 2.07           \\\hline
\multirow{3}{*}{\textbf{shuttle}}  & \textbf{0.005}             & 4.96              & 2.69          & 25.84            & 198.64           & 236.72        & 2.22           \\
                                   & \textbf{0.01}              & 2.95              & 1.18          & 27.07            & 278.99           & 78.96         & 0.99           \\
                                   & \textbf{0.05}              & 1.33              & 0.98          & 1.14             & 2746.8           & 10.37         & 1.37           \\ \bottomrule
\end{tabular}
}
\caption{Algorithm CPU time among dataset collection 4.}
\label{tab:COL4_3}
\end{table}

==> tables/COL4/COL4_table_4.tex <==
\begin{table}[H]
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{cc|cccccc}
\toprule
 \bottomrule
\end{tabular}
}
\caption{Algorithm ARI among dataset collection 4.}
\label{tab:COL4_4}
\end{table}
